On Explaining Confounding Bias

When analyzing large datasets, analysts are often interested in the explanations for surprising or unexpected results produced by their queries. In this work, we focus on aggregate SQL queries that expose correlations in the data. A major challenge that hinders the interpretation of such queries is confounding bias, which can lead to an unexpected correlation. We generate explanations in terms of a set of confounding variables that explain the unexpected correlation observed in a query. We propose to mine candidate confounding variables from external sources since, in many real-life scenarios, the explanations are not solely contained in the input data. We present an efficient algorithm that finds the optimal subset of attributes (mined from external sources and the input dataset) that explain the unexpected correlation. This algorithm is embodied in a system called MESA. We demonstrate experimentally over multiple real-life datasets and through a user study that our approach generates insightful explanations, outperforming existing methods that search for explanations only in the input data. We further demonstrate the robustness of our system to missing data and the ability of MESA to handle input datasets containing millions of tuples and an extensive search space of candidate confounding attributes.

==> background.tex <==
\section{Background and Assumptions}
\label{sec:background}
\yin{The story of the covid cases is interesting, but maybe we need to talk about an application scenario.}


We make the following key assumption, standard in statistics.
The database $\mathcal{T}$ is a uniform sample from a large population (e.g., all
countries in the world, etc.), obtained according
to some unknown distribution $Pr(A)$. 


\paragraph*{Entropy and Mutual Information}
The entropy of an attribute $a \in A$ is $H(a) := -\sum_{v \in Dom(a)}Pr(v) \log(Pr(v))$, where $Pr(v)$ is the
marginal probability and $dom(a)$ denotes the domain of values of $a$. The mutual information of two attributes $a,b \in A$ is defined as $I(a;b) = H(a) + H(b)- H(a;b)$, where $H(a;b)$ is the joint entropy of $a$ and $b$. The conditional mutual information of three attributes $a,b,c \in A$ is
$I(a;b|c) := H(a;c) + H(a;b) - H(a;b;c) - H(c)$. We say that $a$ and $b$ are
conditionally independent $a \independent b | c$, if $I (a; b|c) = 0$.


\brit{here}
Since $Pr(A)$ is unknown, to estimate
the entropy from the database $\mathcal{T}$ we use the Miller-Madow estimator \cite{carlton1969bias}: Hˆ (X) =
P
x∈ΠX (D) F (x) log F (x) +
m−1
2n
, where F (x) =
1
n
P
a∈D 1a[X]=x
(the empirical distribution function) andm = |ΠX(D)|
is the number of distinct elements of X. We refer to the sample
estimate of I (X; Y|Z) as ˆI (X; Y|Z).




\paragraph*{Causal DAGs}. A causal DAG $G = \langle V, E \rangle$ is a directed graph whose nodes are
the set of attributes, i.e., $V = A$ and whose edges $E$ capture all
potential causal relationships between the attributes \cite{pearl2013direct,pearl2009causality}. Given an attribute $a$, we denote by $PA(a)$
the set of parents of $a$. If there exists a directed
path from $a$ to $b$ in $G$ we say that $a$ is an ancestor or a cause of
$a$, and say that $b$ is a descendant or an effect of $a$. A probability
distribution $Pr(A)$ is called causal, or DAG-isomorphic, if there exists
a DAG $G$ with nodes $A$ that captures precisely its independence
relations \cite{pearl2009causality}. Throughout this paper we
assume Pr is DAG-isomorphic.

